PoC-Gym: Towards More Reliable LLM-Assisted Proof-of-Concept Exploit Generation

Recently Large Language Models (LLMs) have been used in security-related tasks, including generating proof-of-concept (PoC) exploits. Several LLM-assisted approaches have been proposed; they typically generate PoCs from vulnerability descriptions and use additional guidance. But, such approaches are often ineffective because the signals-such as printed markers, generated files, or runtime side effects-that they use for validation may not imply that the vulnerability is triggered. Research for more reliable PoC generation is in need but yet remains challenging. We propose PoC-Gym, a pipeline for LLM-based PoC generation for Java security vulnerabilities. PoC-Gym uses both static and dynamic information, e.g., CVE-tailored prompts, static traces, and coverage-based feedback, and iteratively generates PoC candidates. Each candidate goes through a series of validations: whether the execution is complete, manifests a success signal, and reaches the sink of the target trace. We evaluate PoC-Gym using 20 Java CVEs. Across 338 runs, 116 candidates pass PoC-Gym's runtime validation and 65 candidates pass post-hoc validation against the ground-truth vulnerable locations, covering 12 of the 20 CVEs. On the 14-CVE overlap with FaultLine, the strongest PoC-Gym configuration is post-hoc valid for 8 CVEs, while FaultLine reports success for 5 CVEs under its original evaluation criterion. But, given the complexity of PoC generation, PoC-Gym also generates many runtime-valid but post-hoc-invalid PoCs. To better understand how to achieve more reliable PoC generation, we present an in-depth analysis of such PoCs and identify common sources of failures. We believe that our work provides insights for future research.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto
